Variational Inference for Gaussian Process with Panel Count Data

We present the first framework for Gaussian-process-modulated Poisson processes when the temporal data appear in the form of panel counts. Panel count data frequently arise when experimental subjects are observed only at discrete time points and only the numbers of occurrences of the events between subsequent observation times are available. The exact occurrence timestamps of the events are unknown. The method of conducting the efficient variational inference is presented, based on the assumption of a Gaussian-process-modulated intensity function. We derive a tractable lower bound to alleviate the problems of the intractable evidence lower bound inherent in the variational inference framework. Our algorithm outperforms classical methods on both synthetic and three real panel count sets.

==> introOld.tex <==
\paragraph{Introduction of panel count data.}

Count data frequently arise as outcomes of an underlying \emph{count process} in continuous time. A classical example for a count process is the number of accidents on a particular stretch of road during a fixed time interval. Count data can generally be classified into two types. One is from the studies that monitor subjects continuously and thus provide information on the times of all occurrences of the events. These data are usually referred to as \emph{recurrent event data}. The other type is the so-called \emph{panel count data}, which is the focus of our paper. Under this framework, subjects are examined or observed only at discrete time-points and thus give only the numbers of occurrences of the events between observation times. 

By studying the relationships between the underlying count process, the most noticeable being the homogeneous Poisson process, and the resulting probability models for event counts, enables us to acquire better understanding of the conditions under which a given count distribution is appropriate. For example, the classical Poisson process, resulting in the Poisson distribution for the number of counts during a fixed time interval, requires independence and constant probabilities  for occurrence of successive events, an assumption that appears to be quite restrictive in most applications to machine learning applications as well as elsewhere.

Many observed phenomena, from the changing weather systems to medical data such as a patient's blood pressure or temperature, are distinguished by quantities that vary over time. Precisely, the times of events are not observed precisely; and in most practical cases, they can never be observed ‘exactly’ in a continuous time setting. In the context of this paper, we are generally confronted with the problem that we \textit{do not} observe directly the event times, but \textit{do} observe the number of events in a time frame.

Our data inherits this phenomenon in which the value of an observation is only partially known. In our case, the exact times at which events happen are \textit{not observable}. Formally, panel count data arises when the event of interest cannot be directly observed but is only known to have occurred during an interval of time.  Count data framework, investigate properties of $N(T)$ where $N(T)$ describe the number of occurrences during the interval $(0,T)$ for a given $T$. In such cases, the only information we have is the number of events over a given interval, but the times at which the event happens are not known. Some notable examples include medical trials: the subject may be observed only periodically, rather than assessed in a continuous fashion. The medical practitioners would report the \emph{number} of vomits per day rather than the \emph{precise timings} at which the vomiting occurs within that day for patients.


In the present text, we give insights into the modelling of panel data for the Gaussian process modulated Poisson processes model as proposed in asdf \cite{}. To carry out inference in this setting, we use match the moments of the varitional distribution by spelling out solutions for some expressions of the number of events over a fixed time interval $[0,T]$.

\paragraph{Purpose of this paper.}
The present paper treats situations where individuals experience repeated events, and data on an individual consist of an observed point process whose intensity is driven by a certain specificities of Gaussian Process, along with concomitant covariates. In the types of applications intended here, a fairy large number of individuals is observed over fairly short periods of time. Such data arise in areas such as reliability (e.g., Ascher and Feingold
1984; Crow 1974), medicine (e.g., Bartoszynski, Brown, McBride, and Thompson 1981; Gail, Santner, and Brown 1980), and economics and sociology (e.g., Heckman and Singer 1985, sec. 7; Tuma and Hannan 1984, secs. 2.3 and 8.1). For example, in a reliability context the individual might be a system or piece of equipment, the events in question system failures, and the covariates factors describing the system or the environment in which it operates.


The Poisson model provides the main instrument for modeling count time series data. However other
distributional assumptions may be used instead; the most natural among other candidates being the
negative binomial distribution. Regardless of the chosen distribution, we will review mostly models
that fall under the framework of generalized linear models for time series. This class of models and
the maximum likelihood theory provide a systematic framework for the analysis of quantitative as well
as qualitative time series data. Indeed, estimation, diagnostics, model assessment, and forecasting are
implemented in a straightforward manner, where the computation is carried out by a number of existing
software packages.


Many observed phenomena, from the changing weather systems to medical data such as a patient's blood pressure or temperature, are distinguished by quantities that vary over time. In many situations, the times of events are not observed extremely precisely; and in most practical cases, they can never be observed ‘exactly’ in a continuous time settting. In the context of point processes, we are generally confronted with the problem that we \textit{do not} observe directly the event times, but \textit{do} observe the number of events in a time frame.

Associated with the this phenomenon is known as \textit{interval censoring}. Censoring is a phenomenon in which the value of an observation is only partially known. In our case,  the times at which events happen are \textit{censored}.  Formally, interval censored data arises when the event of interest cannot be directly observed but is only known to have occurred during an interval of time. In such cases, the only information we have is the number of events over a given interval, but the times at which the event happens are not known. Some notable examples include medical trials: the subject may be observed only periodically, rather than assessed in a continuous fashion. The medical practitioners would report the \emph{number} of vomits per day rather than the \emph{precise timings} at which the vomitting occurs within that day for patients.


In the present text, we give insights on the modelling of interval censored data for the gaussian process modulated poisson processes model as proposed in \textcolor{red}{to cite}. To carry out inference in this setting, we use match the moments of the varitional distribution by spelling out solutions for some expressions of the number of events over a fixed time interval $[0,T]$. 


Review of traditional models for panel count data.
Take classical feller or whatever

Show a figure of panel count data here.

Review of model for intensity estimation from complete data.

Introduction to this work

Contribution

Questions for discussion with H. Ding
\textcolor{red}{are you modelling many individuals, or just one individuals?}\\
textcolor{blue}{can you state just one or two reasons why GPR beats the model of comparison? - i want to try generalize that statement in the introduction}


